Zero-Shot Detection of Machine-Generated Codes

This work proposes a training-free approach for the detection of LLMs-generated codes, mitigating the risks associated with their indiscriminate usage. To the best of our knowledge, our research is the first to investigate zero-shot detection techniques applied to code generated by advanced black-box LLMs like ChatGPT. Firstly, we find that existing training-based or zero-shot text detectors are ineffective in detecting code, likely due to the unique statistical properties found in code structures. We then modify the previous zero-shot text detection method, DetectGPT (Mitchell et al., 2023) by utilizing a surrogate white-box model to estimate the probability of the rightmost tokens, allowing us to identify code snippets generated by language models. Through extensive experiments conducted on the python codes of the CodeContest and APPS dataset, our approach demonstrates its effectiveness by achieving state-of-the-art detection results on text-davinci-003, GPT-3.5, and GPT-4 models. Moreover, our method exhibits robustness against revision attacks and generalizes well to Java codes. We also find that the smaller code language model like PolyCoder-160M performs as a universal code detector, outperforming the billion-scale counterpart. The codes will be available at https://github.com/ Xianjun-Yang/Code_detection.git

==> tables/main2.tex <==
\begin{table*}[htbp]
\centering
\caption{Overall comparison of different methods and datasets. The TPR is calculated at 1\% FPR. \textit{w/o P} means the golden prompt is unknown. $K$ in DetectGPT represents the number of perturbations.
}\label{tab:overall} 
\resizebox{0.96\textwidth}{!}
{
\begin{tabular}{lcccccccc}
\toprule
Datasets & \multicolumn{2}{c}{CodeContests} & \multicolumn{2}{c}{HumanEval} & \multicolumn{2}{c}{HumanEval-X} & \multicolumn{2}{c}{Avg.} \\% Mixed-all
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}  
Method & AUROC & TPR & AUROC & TPR & AUROC & TPR & AUROC & TPR  \\
\midrule
%%%%%%%%% GPT-4-0314
\multicolumn{9}{c}{\done  \texttt{GPT-4-0314} }\\
\midrule
GPTZero \cite{GPTZero} & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.0 & 00.00 \\
OpenAI \cite{AITextClassifier} & -- & -- & -- & -- & -- & -- & -- & -- \\
\hline
DetectGPT \cite{mitchell2023detectgpt} & -- & -- & -- & -- & -- & -- & -- & -- \\
DNA-GPT \cite{yang2023dna} & -- & -- & -- & -- & -- & -- & -- & -- \\
\hline
\methodname~, $K$=20, $\gamma$=0.7 & -- & -- & -- & -- & -- & -- & -- & -- \\
\qquad $K$=10, $\gamma$=0.5 & -- & -- & -- & -- & -- & -- & -- & -- \\
\qquad $K$=10, $\gamma$=0.5 & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule
\multicolumn{9}{c}{\done  \texttt{GPT-3.5-turbo}} \\
\midrule

%%%%%%%%% GPT-3.5
GPTZero & -- & -- & -- & -- & -- & -- & -- & -- \\
OpenAI & -- & -- & -- & -- & -- & -- & -- & -- \\
\hline
DetectGPT \cite{mitchell2023detectgpt} & -- & -- & -- & -- & -- & -- & -- & -- \\
DNA-GPT \cite{yang2023dna} & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule
DetectGPT4Code, $K$=20, $\gamma$=0.7 & -- & -- & -- & -- & -- & -- & -- & -- \\
DetectGPT4Code, $K$=20, $\gamma$=0.5 & -- & -- & -- & -- & -- & -- & -- & -- \\
DetectGPT4Code, $K$=10, $\gamma$=0.5 & -- & -- & -- & -- & -- & -- & -- & -- \\
DNA-GPT4Code, $K$=10, $\gamma$=0.5 & -- & -- & -- & -- & -- & -- & -- & -- \\

\bottomrule
\end{tabular}
}
\end{table*}


\begin{table*}[htbp]
\centering
\resizebox{0.96\textwidth}{!}
{
\begin{tabular}{lcccccccc}
\toprule
Datasets & \multicolumn{2}{c}{CodeContests} & \multicolumn{2}{c}{HumanEval} & \multicolumn{2}{c}{HumanEval-X} & \multicolumn{2}{c}{Avg.} \\% Mixed-all
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}  
Method & AUROC & TPR & AUROC & TPR & AUROC & TPR & AUROC & TPR  \\
\midrule
%%%%%%%%% GPT-4-0314
\multicolumn{9}{c}{\done  \texttt{GPT-4-0314} }\\
\midrule
GPTZero \cite{GPTZero} & 67.68 & 00.00 & 23.98 & 3.65 & 36.49 & 7.93 & 00.0 & 00.00 \\
OpenAI \cite{AITextClassifier} & 48.34  & -- & 70.08 & 34.15 & 34.05 & 9.14 & -- & -- \\
\hline
DetectGPT \cite{mitchell2023detectgpt} & 56.30 & -- & -- & -- & -- & -- & -- & -- \\
DNA-GPT, K=15, 20, $\gamma$=0.7, 0.5 \cite{yang2023dna} & 78.27 & 30.33 & 53.09 & 8.54 & -- & -- & -- & -- \\
\hline
DetectGPT4Code, $K$=120, $\gamma$=0.9, $m$=12 & \textbf{86.01} & 62.75 & -- & -- & -- & -- & -- & -- \\
\qquad $K$=10, $\gamma$=0.5 & -- & -- & -- & -- & -- & -- & -- & -- \\
%\qquad $K$=10, $\gamma$=0.5 & -- & -- & -- & -- & -- & -- & -- & -- \\

DNA-GPT4Code, $K$=10, $\gamma$=0.5 & -- & -- & -- & -- & -- & -- & -- & -- \\
\qquad $K$=10, $\gamma$=0.5 & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule
\multicolumn{9}{c}{\done  \texttt{GPT-3.5-turbo}} \\
\midrule

%%%%%%%%% GPT-3.5
GPTZero & 58.94 & -- & 23.98 & 3.65 & 28.38 & 12.20 & -- & -- \\
OpenAI & 64.21 & -- & 90.64 & 66.46 & 24.84 & 3.05 & -- & -- \\
\hline
DetectGPT & -- & -- & -- & -- & -- & -- & -- & -- \\
DNA-GPT, K=10, 20, $\gamma$=0.5 & 70.84 & 23.53 & 65.95 & 11.58 & -- & -- & -- & -- \\
\midrule
DetectGPT4Code, $K$=20, $\gamma$=0.7 & -- & -- & -- & -- & -- & -- & -- & -- \\
\qquad, $K$=20, $\gamma$=0.5 & -- & -- & -- & -- & -- & -- & -- & -- \\
%\qquad, $K$=10, $\gamma$=0.5 & -- & -- & -- & -- & -- & -- & -- & -- \\

DNA-GPT4Code, $K$=10, $\gamma$=0.5 & -- & -- & -- & -- & -- & -- & -- & -- \\
\qquad $K$=10, $\gamma$=0.5 & -- & -- & -- & -- & -- & -- & -- & -- \\

\midrule
\multicolumn{9}{c}{\doneWhite \texttt{LLaMa-13B(White-box)} } \\
\midrule
GPTZero \cite{GPTZero} & -- & 00.00 & 79.88 & 51.22 & -- & -- & 00.0 & 00.00 \\
OpenAI \cite{AITextClassifier} & --  & -- & 49.27 & 33.54 & -- & -- & -- & -- \\
\hline
DetectGPT \cite{mitchell2023detectgpt} & -- & -- & -- & -- & -- & -- & -- & -- \\
DNA-GPT, K=15, 20, $\gamma$=0.7, 0.5 \cite{yang2023dna} & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule
DetectGPT \cite{mitchell2023detectgpt}, $K$=20 & -- & -- & -- & -- & -- & -- & -- & -- \\ 
\qquad $K$=100  & -- & -- & -- & -- & -- & -- & -- & -- \\ \hline
\methodname~, $K$=20, $\gamma$=0.7 & -- & -- & -- & -- & -- & -- & -- & -- \\
\qquad $K$=10, $\gamma$=0.5, & -- & -- & -- & -- & -- & -- & -- & -- \\

\qquad $K$=10, $\gamma$=0.5, w/o P & -- & -- & -- & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabular}

}
\caption{Overall comparison of different methods and datasets. The TPR is calculated at 10\% FPR (corresponding to 10 to 15 instances), considering a total of around 100 to 150 testing instances for each dataset. $K$ in DetectGPT represents the number of perturbations. Programming language for CodeContests, HumanEval and HumanEval-X is Python, Python, and Java, respectively.
}\label{tab:overall} 
\end{table*}


